Approximate Newton-based statistical inference using only stochastic gradients

We present a novel statistical inference framework for convex empirical risk minimization, using approximate stochastic Newton steps. The proposed algorithm is based on the notion of finite differences and allows the approximation of a Hessian-vector product from first-order information. In theory, our method efficiently computes the statistical error covariance in $M$-estimation, both for unregularized convex learning problems and high-dimensional LASSO regression, without using exact second order information, or resampling the entire data set. We also present a stochastic gradient sampling scheme for statistical inference in non-i.i.d. time series analysis, where we sample contiguous blocks of indices. In practice, we demonstrate the effectiveness of our framework on large-scale machine learning problems, that go even beyond convexity: as a highlight, our work can be used to detect certain adversarial attacks on neural networks.

==> cmp-stat-inf-sgd-avg-spnd.tex <==

\section{Comparison of stochastic proximal Newton descent and SGD averaging for statistical inference}
\label{sec:cmp-stat-inf-sgd-avg-spnd}


Here, we present a heuristic argument demonstrating that stochastic proximal Newton descent has smaller variance than SGD averaging for statistical inference. 
Our argument use simplified interpretations fro stochastic proximal Newton descent and SGD. 
There are fewer random components in stochastic proximal Newton descent compared than SGD averaging, 
thus stochastic proximal Newton descent has a smaller estimation variance. 

A more rigorous comparison requires a better understanding of Edgeworth expansions in stochastic  approximation (e.g. \cite{dippon2008asymptotic, dippon2008edgeworth}), 
which would also allow for a better comparison with resampling methods such as bootstrap and subsampling \cite{hall2013bootstrap}. 

Our goal here is to approximate the distribution $\Norm(0, H^{-1} G H^{-1} )$, 
using a sample $g \sim \Norm(0, G)$. 
Note that this is straightforward if we can exactly compute $H^{-1}$ and use $H^{-1}g$ (as in vanilla Newton method), 
whose distribution is exactly  $\Norm(0, H^{-1} G H^{-1} )$. 

When we cannot compute $ H^{-1} $ due to space or time limitations, we can use stochastic gradient methods to approximate $\Norm(0, H^{-1} G H^{-1} )$. 
It is a well known fact \cite{hardt-blog-gd-zen} that full gradient descent can be viewed as deterministically computing $H^{-1}$ using the identity $H^{-1}= \eta \sum_{i=0}^\infty (I-\eta H)^i$.
And stochastic gradient methods can be viewed as an unbiased estimate of $H^{-1}$, as described below.  


\paragraph{Stochastic proximal Newton descent} 
The stochastic proximal Newton descent statistical inference method can be interpreted as using the recursion 
\begin{align}
v_{t+1} = (I - \tau_t H_t) v_t + \tau_t v_0 , 
\end{align}
where $v_0 \sim \Norm(0, G)$ and $H_t$ is independently sampled from $\{H_{(1)}, H_{(2)}, \dots, H_{(n)}\}$ where $\frac{1}{n} \sum_{i=1}^n H_{(i)} = H$, 
and computing the covariance of $\frac{1}{t} \sum_{i=1}^t v_i$. 
Here $v_0$ and all $H_i$ are independent. 
%We can calculate that 
%\begin{align}
%\Exp[ (\frac{1}{t} \sum_{i=1}^t v_i) (\frac{1}{t} \sum_{i=1}^t v_i)^\top ] = .  
%\end{align}


\paragraph{SGD averaging}
The SGD averaging statistical inference method \cite{li2017statistical, chen2016statistical} uses averages of consecutive SGD iterates. 
Each update is given by 
\begin{align}
\theta_{t+1} = \theta_t - \eta_t \left( \frac{1}{S} \sum_{j \in I_t} \nabla f_j(\theta_t) \right) , 
\end{align}
where $I_t$ are $S$ indices sampled with replacement from $[n]$. 
And we use $\sqrt{S \cdot t} \left( ( \frac{1}{t} \sum_{i=1}^t \theta_i) - \htheta \right)$ for statistical inference. 
It can be interpreted as using the recursion 
\begin{align}
v_{t+1} = (I - \eta_t H_t) v_t + \eta_t g_t , 
\end{align}
where each $g_i \sim \Norm(0, G)$ is i.i.d. and $H_t$ is sampled from $\{H_{(1)}, H_{(2)}, \dots, H_{(n)}\}$ where $\frac{1}{n} \sum_{i=1}^n H_{(i)} = H$, 
and computing the covariance of $\frac{1}{\sqrt{t}} \sum_{i=1}^t v_i$. {\blue{this is not entirely correct, $H_i$, $g_i$ are correlated}}
%We can calculate that 
%\begin{align}
%\Exp[ (\frac{1}{\sqrt{t}} \sum_{i=1}^t v_i) (\frac{1}{\sqrt{t}} \sum_{i=1}^t v_i)^\top ] = .
%\end{align}



==> discussion.tex <==


\section{Discussion}
\label{sec:discussion}


Our approximate Newton-based statistical inference procedure provides a general and flexible framework for {\em simultaneous} point estimation and statistical inference.
\Cref{alg:stat-inf-spnd} is the ``cheapest'' version, where 
\TODO{plug in algorithms} \cite{toulis2017asymptotic,harikandeh2015stopwasting,loshchilov2015online,daneshmand2016starting}

%A better understanding of concentration and Edgeworth expansion \cite{dippon2008asymptotic,dippon2008edgeworth} in stochastic approximation would give stronger guarantees for our algorithms. 


==> high-dim-stat-inf-cheap-sgd-no-proof.tex <==



\section{High dimensional linear regression statistical inference by solving stochastic Newton steps using proximal SGD}
\label{sec:high-dim-cheap-sgd-no-proof:stat-inf:proximal-sgd}

Here, we present  a less computationally expensive algorithm  for statistical inference in high dimensional linear regression using proximal SGD to solve proximal Newton steps, which doesn't use full gradients, is given in \Cref{sec:high-dim-cheap-sgd-no-proof:stat-inf:proximal-sgd}.
However, existing techniques for proximal SGD \cite{atchade2017perturbed} and SGD \cite{moulines2011non} only guarantees $\ell_2$ bounds, 
and a better understanding of concentration and Edgeworth expansions \cite{dippon2008asymptotic,dippon2008edgeworth} in stochastic approximation for $\ell_\infty$ bounds is required for provable guarantees in the high dimensional setting. 







==> macros_colt.tex <==
%\usepackage{algpseudocode}
%\usepackage{algorithm}
%\usepackage{amsmath, amssymb, amsthm, amsfonts}
%\usepackage{undertilde}
%\usepackage{float}
\usepackage{graphicx}
%\usepackage{caption}
%\usepackage{subcaption}
%\usepackage{natbib}
\usepackage{color}
%\usepackage{bbm}
%\usepackage{epstopdf}
\usepackage{wrapfig, framed}
\usepackage{mathrsfs}


% https://tex.stackexchange.com/questions/53690/tagging-under-an-equation-using-underbrace
\makeatletter
\newcommand{\mytag}[2]{%
  \text{#1}%
  \@bsphack
  \begingroup
    \@onelevel@sanitize\@currentlabelname
    \edef\@currentlabelname{%
      \expandafter\strip@period\@currentlabelname\relax.\relax\@@@%
    }%
    \protected@write\@auxout{}{%
      \string\newlabel{#2}{%
        {#1}%
        {\thepage}%
        {\@currentlabelname}%
        {\@currentHref}{}%
      }%
    }%
  \endgroup
  \@esphack
}
\makeatother



\newcommand{\polylog}{{\operatorname{polylog}}}

\newcommand{\bbeta}{{\bar{\beta}}}

\newcommand{\MAP}{{\mathrm{MAP}}}

\def\tsum{{\mathop{\textstyle \sum }}}

% Theorem defintions
%\newtheorem{proposition}{Proposition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{definition}{Definition}


\newcommand{\Exp}{{\operatorname{\mathbb{E}}}}
\newcommand{\Prob}{{\operatorname{\mathbb{P}}}}
\newcommand{\Var}{{\operatorname{Var}}}
\newcommand{\Norm}{\mathcal{N}}
%\newcommand{\bfSigma}{{\boldsymbol\Sigma}}
%\newcommand{\bfmu}{{\boldsymbol\mu}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\ttheta}{\theta^{\star}}
\newcommand{\ebeta}{\hat{\beta}}
\newcommand{\tibeta}{\tilde{\beta}}
\newcommand{\etheta}{\hat{\theta}_{\lambda_n}}
\newcommand{\errvec}{\hat{\Delta}}
\newcommand{\poprisk}{\overline{\calL}}
\newcommand{\emprisk}{\calL}
\newcommand{\reg}{\mathcal{R}}
\newcommand{\supp}{\operatorname{supp}} 
\newcommand{\half}{\frac{1}{2}}
\newcommand{\blue}[1]{{\color{blue}{#1}}}

\newcommand{\Cov}{\operatorname{Cov}}

\newcommand{\ltynorm}[2]{\| {#1} \|_{#2}}
\newcommand{\er}{\mathcal{E}} % excess risk
\newcommand{\ern}{\mathcal{E}_n} % excess risk
\newcommand{\hbeta}{\widehat{\beta}}
\newcommand{\htheta}{\widehat{\theta}}
\newcommand{\btheta}{\bar{\theta}}
\newcommand{\tbeta}{\tilde{\beta}}
\newcommand{\hSigma}{\hat{\Sigma}}
\newcommand{\Loss}{\mathcal{L}}
\newcommand{\hf}{\hat{f}}

\newcommand{\sign}{\operatorname{sign}}
\newcommand{\idONE}{\operatorname{\mathbf{1}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}

\newcommand{\utilde}[1]{\underset{\sim}{#1}}

\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}

% space saving
%\input{space_saver}
% useful shortcuts

% assorted
\usepackage{url}
\usepackage{xspace}
\usepackage{comment}
\usepackage{color}
\usepackage{afterpage}

%\newcommand{\Real}{\mathbb{R}}

\newcommand{\TODO}[1]{{\blue{\textbf{TODO} #1}}}



==> regularized-local.tex <==




\section{General regularized M-estimation}
\label{sec:general-regularized-m-est}

Here we present a local stochastic proximal Newton descent algorithm for statistical inference in general regularized M-estimation. 
%Suppose that we observe $n$ i.i.d. data points $X_1, X_2, \dots, X_n$, 
%and we have a loss function $\ell(X; \theta)$. 
Suppose that we have a $p$-dimensional regularized problem
\begin{align}
\htheta  = \arg \min_{\theta \in \Real^p}  f(\theta) + \lambda R(\theta) ,  
\end{align}
%where $f_i(\theta) = \ell(X_i;\theta)$, 
%and we denote $f(\theta) = \frac{1}{n} \sum_{i=1}^n f_i(\theta)$. 
where $f$ is a general cost function and $R$ is a regularizer. 

%\subsection{Statistical asymptotic normality}
%
%\subsection{Statistical inference using stochastic proximal Newton descent}

%\subsection{Gaussian graphical model high dimensional statistical inference}





==> spnd-opt.tex <==


\section{Stochastic proximal Newton descent optimization}
\label{append:sec:spnd-opt}

\subsection{Unregularized M-estimation}
\label{append:sec:spnd-opt:subsec:unregularized-m-est}

Here we present a stochastic proximal Newton descent  optimization algorithm using stochastic gradients, which is analogous to \Cref{alg:stat-inf-spnd}. 
Note that this can be viewed as a generalization of SVRG \cite{johnson2013accelerating} (\Cref{append:sec:svrg-intuition}). 



\subsection{LASSO linear regression}

Here we present a stochastic proximal Newton descent optimization algorithm for solving the modified LASSO problem in \eqref{eq:lasso-mod-cov}. 



